Model checking: the interval way

[...] The most famous model checking (MC) techniques were developed from the late 80s, bearing in mind the well-known "point-based" temporal logics LTL and CTL. However, while the expressiveness of such logics is beyond doubt, there are some properties we may want to check over system models that are inherently "interval-based" and thus cannot be expressed by point-based temporal logics, e.g., "the proposition p has to hold in at least an average number of system states in a given computation sector". Here interval temporal logics (ITLs) come into play, providing an alternative setting for reasoning about time. Such logics deal with intervals, instead of points, as their primitive entities: this feature gives them the ability of expressing temporal properties, such as actions with duration, accomplishments, and temporal aggregations, which cannot be dealt with in standard point-based logics. The Halpern and Shoham's modal logic of time intervals (HS) is one of the most famous ITLs: it features one modality for each of the 13 possible ordering relations between pairs of intervals, apart from equality. In this thesis we focus our attention on MC based on HS, in the role of property specification language, for which a little work has been done if compared to MC for point-based temporal logics. We study the complexity of such problem considering different system models, and we also compare the expressive power of HS to that of LTL, CTL and CTL* in MC. [...]

==> Chaps/Intro/TBD_introINFOR.tex <==
% \setcounter{chapter}{-1}

% \chapter[An informal introduction (and some trifles)]{An informal introduction\\ (and some trifles)}
% \label{chap:introINFOR}
% \minitoc\mtcskip

%
%
% \footnote{Yes, in this section I often use the ``I'' pronoun, and a half-serious style. If the reader doesn't like it, I want to reassure her: all the next sections follow the certainly more familiar, scientific impersonal style.
% A reviewer may safely skip this chapter: I can't blame her if she doesn't want to listen to me talking nonsense :)}

% I don't want to bore you with the details. 
% The reliability of IT systems is a key issue, starting from the system design process!
% System verification is used to establish that the design or product under consideration possesses certain properties. Specification: what the system has to do and what not; defect: the system does not fulfill one of the specification properties.

% [\dots] Computer science is relatively new; as a
% consequence when the software production activity
% begins, we usually get wrong budget estimates,
% production periods are wrongly calculated, products are
% often delivered with unexpected behaviours, or with
% operational failures, or with scarce security and safety
% features.
% If a building contractor made incorrect estimates,
% built studio apartments in place of penthouses or building
% that collapsed after some months, he would not survive.
% An enterprise that built an automobile which broke down
% twice a day would go bankrupt. A computer software
% that makes your PC halt twice a day is normally sold,
% bought and used.

% «The computer is such a complex machine that it's not strange that sometimes it doesn't work;
% conversely, it's a miracle it usually works fine!»

% The two de facto reference textbooks---the ``older''~\cite{CGP02} and the more modern~\cite{Baier2008}---adopted in almost all graduate courses on model checking, define it respectively as:
% \begin{quotation}
% [\dots] an automatic technique for verifying finite state concurrent systems. 
% It has a number of advantages over traditional approaches that are based on
% simulation, testing, and deductive reasoning. 
% The method has been used successfully in
% practice to verify complex sequential circuit designs and communication protocols. 
% [\dots]
% The procedure
% normally uses an exhaustive search of the state space of the system to determine if some
% specification is true or not. Given sufficient resources, the procedure will always terminate
% with a yes/no answer.
% \end{quotation}
% %
% and
% \begin{quotation}
% [\dots] a prominent formal-verification technique for assessing functional properties of information and communication systems. Model checking
% requires a [finite-state] model of the system under consideration and a desired [formally specified] property and systematically checks whether or not the given model satisfies this property. Typical properties
% that can be checked are deadlock freedom, invariants, and request-response properties.
% Model checking is an automated technique to check the absence of errors (i.e., property
% violations) and alternatively can be considered as an intelligent and effective debugging
% technique. It is a general approach and is applied in areas like hardware verification and
% software engineering.
% \end{quotation}

%  Note that the property specification
% prescribes what the system should do, and what it should not do, whereas the model
% description addresses how the system behaves.

% I've often been asked if I don't ever get bored while studying the complexity of fragments of HS by «just adding something and removing something else». Well, the answer is (in general) «No!».%
% \footnote{Clearly, the exception is when we don't manage to reach some results we expect\dots}
% As I (we) will try to persuade the reader of, is that, in spite of being the problem pretty much the same---apart from the specific fragments under consideration---the techniques we employ are always different and tailored to the specific situation. 
% Obviously this is, on one hand, fun, 
% on the other, sometimes pretty annoying, as you can hardly re-use what you have already done in a similar context. (Elenco high-level: small models, contrazioni, circuiti...)

% So we are left with three open problems. We may as well put up with two of them,
% but one really gets on our nerves.
% It's the model checking problem for the fragment BE.
% BE is known to be the devil, the hard core to kill of HS.
% Undecidable as for its satisfiability problem, BE is known to be EXPSPACE-hard in model checking, but we only 
% managed to craft a decision algorithm having nonelementary complexity\dots 
% To try to close such complexity gap, or perhaps I should say, such abyss, we ended up falling in it\dots
% The problem is still there, waiting for somebody to solve it. As one of us suggested,
% BE model checking should perhaps be regarded as a difficult challenge, to possibly overcome in the long term.
% So charmingly elegant and easy to explain, it may draw the attention of other people and researchers I feel compelled to warn:
% BE may keep them awake at night, unless taken in small doses.


==> Chaps/Timelines/MCTimelinesOLD.tex <==
\section{Model Checking \MITL\ Specifications over Timelines} \label{sec:modelchecking}

In this section, we outline how to model check real-time systems, described in terms of timelines,
using the logic \MITL\ (Metric Interval Temporal Logic)~\cite{Alur:1996} as the property specification language.
%
Henceforth, $\Prop$ denotes a set of proposition letters.
Two intervals $I$ and $I'$ are said to be \emph{adjacent} iff the right endpoint of $I$ equals the left endpoint of $I'$,
and either $I$ is right-closed and $I'$ left-open, or $I$ is right-open and $I'$ left-closed.

\MITL\ formulas are
defined by the grammar $\psi ::= p\mid \neg \psi \mid \psi \wedge \psi\mid \psi \UI \psi $,
where $p\in\Prop$ and $I\in \mathbb{I}(\Nat\cup\{+\infty\})$, at the subscript of $\mathsf{U}$, is nonsingular.
%
\MITL\ formulas are interpreted over timed state sequences.
A \emph{timed state sequence} $(\overline{s},\overline{I})$ is given by an infinite sequence of states $\overline{s}=s_1s_2s_3\cdots$, where $s_i\subseteq \Prop$, and an infinite
sequence of time intervals $\overline{I}=I_1 I_2 I_3\cdots$, where $I_i \in \mathbb{I}(\RealP\cup\{+\infty\})$,
such that $(i)$~$I_1$ is left closed and 0 its left endpoint, $(ii)$~for all $i\geq 1$, $I_i$ and $I_{i+1}$ are adjacent, and $(iii)$~for all $t\in\RealP$, $t \in I_j$ for some $j\geq 1$.

For $t\in\RealP$, $(\overline{s},\overline{I})^t$ denotes the timed state sequence $(\overline{s}',\overline{I}')$ where,
assuming $t \in I_j$ for a $j\geq 1$, we have
$\overline{s}'\!=\!s_j s_{j+1}\cdots$, $\overline{I}'\!=\!I_j' I_{j+1}'\cdots $, with $I_i'\!=\!\{t'\!-\! t \!\mid\!  t'\in I_i ,\, t'-t\geq 0\}$ for all $i\geq j$.

The satisfaction relation $(\overline{s},\overline{I})\models \psi$ is defined as (we omit the clauses for Boolean operators):
$(i)$~$(\overline{s},\overline{I})\models p$ iff $p\in s_1$;
$(ii)$~$(\overline{s},\overline{I})\models \psi_1 \UI \psi_2$ iff, for some $t\in I$, $(\overline{s},\overline{I})^t\models \psi_2$ and for all $0<t'< t$, $(\overline{s},\overline{I})^{t'}\models \psi_1$.

The following results appeared in~\cite{Alur:1996} (Theorem~4.4.1 and 4.5.2).
Let $\psi$ be a \MITL\ formula, where $N$ is the number of subformulas of $\psi$, and $K$ the largest integer constant appearing in $\psi$:
$(i)$~we can build a \TA\ $\mathcal{A}_\psi$ accepting the set of timed state sequences $(\overline{s},\overline{I})$ that satisfy $\psi$, with $O(2^{N\cdot K})$ states and $O(N\cdot K)$ clocks. Thus deciding its emptiness requires exponential space.
$(ii)$~If in $\psi$ all intervals at the subscript of $\mathsf{U}$ have the form $[0,a]$, $[0,a)$, $[a,+\infty)$, or $(a,+\infty)$ (such fragment is denoted as $\MITL_{0,\infty}$), it is possible to build a \TA\ $\mathcal{A}_\psi$ accepting the set of sequences $(\overline{s},\overline{I})$ that satisfy $\psi$,
    with $O(2^{N})$ states and $O(N)$ clocks. Deciding its emptiness requires polynomial space.\footnote{In the case of $\MITL_{0,\infty}$ formulas, we may also assume that intervals constraining the operator $\mathsf{U}$ have rational bounds, at no increased complexity cost.}

Let us now consider a system description, given as a planning problem $P=(\{x_1,\ldots , x_k\}, \allowbreak S)$.
For every state variable $x_j$, we encode every $v\in V_{x_j}$ by a suitable truth assignment to $\log |V_{x_j}|$ proposition letters $\Prop_j=\{p_{x_j,1},\ldots, p_{x_j,\log |V_{x_j}|}\}$. 
We denote by $\enc(x_j,v)$ the set of letters which are true in the encoding of $v$.
In this way, 
a 
timed $k$-multiword $(\vct{a}_1,\tau_1)(\vct{a}_2,\tau_2)\cdots$
can be considered as the timed state sequence $(\overline{s},\overline{I})$ where, for all $i\geq 1$, $I_i=[\tau_i,\tau_{i+1})$ and
(let $s_0=\emptyset$)
$s_i=(\bigcup_{j=1,\ldots , k,\, \vct{a}_i[j]\neq \epsilon} \enc(x_j,\vct{a}_i[j]))\cup (\bigcup_{j=1,\ldots , k,\, \vct{a}_i[j]=\epsilon} s_{i-1}\cap \Prop_j)$.

Now, given a system model $P=(\{x_1,\ldots , x_k\},S)$ and a property specification (\MITL\ formula) $\psi$, we have to decide whether or not $\TLang(\tilde{\mathcal{A}})\subseteq \TLang(\mathcal{A}_\psi)$, where $\tilde{\mathcal{A}}$ is the \TA\ for $P$ (Proposition~\ref{prop:LtA}).
For the purpose we check whether $\TLang(\tilde{\mathcal{A}})\cap \TLang(\mathcal{A}_{\neg \psi})= \emptyset$, by making the product automaton 
$\tilde{\mathcal{A}}\times \mathcal{A}_{\neg \psi}$, and checking for its emptiness. The size of $\tilde{\mathcal{A}}\times \mathcal{A}_{\neg \psi}$ is polynomial in those of $\tilde{\mathcal{A}}$ and $ \mathcal{A}_{\neg \psi}$.
The next result follows.

\begin{theorem}
The MC problem for \MITL\ formulas over timelines is in \EXPSPACE.
It is in \Psp\ for $\MITL_{0,\infty}$.
\end{theorem}

==> Chaps/Timelines/tilingGraph.tex <==
\begin{tikzpicture}[node distance=0 cm,outer sep = 0pt]

%\draw[use as bounding box] (-1,301) rectangle (16,200);

\tikzstyle{cella}=[draw, rectangle,  minimum height=0.7cm, minimum width={width("dddddd")},anchor=south west];
\tikzstyle{dcella}=[draw, rectangle, dashed, minimum height=0.7cm, minimum width={width("dddddd")},anchor=south west];
%
\node[cella] (k-0) at (0,300) {$d^k_0$};
\node[cella] (k-1) [right = of k-0] {$d^k_1$};
\node[cella] (k-2) [right = of k-1] {$d^k_2$};
\node[dcella] (k-3) [right = of k-2] {};
\node[dcella] (k-4) [right = of k-3] {};
\node[dcella] (k-5) [right = of k-4] {};
\node[cella] (k-6) [right = of k-5] {$d^k_{2^n-2}$};
\node[cella] (k-7) [right = of k-6] {$d^k_{2^n-1}$};
%
\node[dcella] (k1-4) [below = of k-4] {};
\node[cella] (k2-4) [below = of k1-4] {$d^{j+1}_i$};
\node[cella] (k3-4) [below = of k2-4] {$d^{j}_i$};
\node[cella] (k4-4) [below = of k3-4] {$d^{j-1}_i$};
\node[cella] (k3-3) [left = of k3-4] {$d^{j}_{i-1}$};
\node[cella] (k3-5) [right = of k3-4] {$d^{j}_{i+1}$};
\node[dcella] (k5-4) [below = of k4-4] {};
%
%\node[cella] (k-0)  {$d^k_0$};
\node[dcella] (1-4) [below = of k5-4] {};
\node[dcella] (1-5) [right = of 1-4] {};
\node[dcella] (1-3) [left = of 1-4] {};
\node[cella] (1-2) [left = of 1-3] {$d^0_2$};
\node[cella] (1-1) [left = of 1-2] {$d^0_1$};
\node[cella] (1-0) [left = of 1-1] {$d^0_0$};
\node[cella] (1-6) [right = of 1-5] {$d^0_{2^n-2}$};
\node[cella] (1-7) [right = of 1-6] {$d^0_{2^n-1}$};
%
 \node [align=left,red](13) [left = of 1-0] {$d_{init}$};
 \node [align=left,red](13) [right = of k-7] {$d_{final}$};
%
\node[cella] (k-k) at (10.9,298) {$d^j_i$};
\node [align=left,red] [left = of k-k] {$[d^j_i]_\Left$};
\node [align=left,red] [right = of k-k] {$[d^j_i]_\Right$};
\node [align=left,red] [below = of k-k] {$[d^j_i]_\Down =$};
\node [align=left,red] [above = of k-k] {$[d^j_i]_\Up$};
%
\node[cella] (k-k-1) at (10.9,296) {$d^{j-1}_i$};
\node [align=left,red] [above = of k-k-1] {$[d^{j-1}_i]_\Up$};
%
\node[dcella] (i-0) [below = of k-0] {};
\node[dcella] (i-1) [below = of i-0] {};
\node[dcella] (i-2) [below = of i-1] {};
\node[dcella] (i-3) [below = of i-2] {};
\node[dcella] (i-4) [below = of i-3] {};
%
\node[dcella] (j-0) [below = of k-7] {};
\node[dcella] (j-1) [below = of j-0] {};
\node[dcella] (j-2) [below = of j-1] {};
\node[dcella] (j-3) [below = of j-2] {};
\node[dcella] (j-4) [below = of j-3] {};

\end{tikzpicture}


==> FrontBackMatter/frontespizio2.tex <==
\thispagestyle{empty}
\tikz[remember picture,overlay] \node[inner sep=0pt,opacity=0.3] at 
(current page.center){\includegraphics[width=0.93\paperwidth%,height=\paperheight
]{Gfx/logouni3}};

\tikz[remember picture,overlay] \node[inner sep=0pt] at 
(current page.center){%inizio minipage
%
\begin{minipage}[c][0.85\paperheight][c]{0.8\paperwidth}

\begin{center}
\textsc{
{\Large Università degli Studi di Udine}
\bigskip 
\hrule
\bigskip
\begin{large}
Dipartimento di Matematica, Informatica e Fisica\\\medskip
Corso di Dottorato in\\ Informatica e Scienze Matematiche e Fisiche\\\bigskip
Ciclo XXXI
\end{large}
}

\vfill

{\LARGE \textsc{Model Checking:}}
\\ \vspace{0.4cm}
{\LARGE \textsc{the Interval Way}}
% \\ \vspace{1cm}
% {\Large \textsc{Model Checking e Logiche Temporali a Intervalli:}}
% \\ \vspace{0.2cm}
% {\Large \textsc{Verificare Proprietà Intervallari delle Computazioni}}
\\ \vspace{1cm}
{\large Tesi di Dottorato}

\vfill

\begin{large}
\begin{flushleft}
Relatore \\ 
prof.\ Angelo MONTANARI\\
\vspace{0.8cm}
\rule{0.6\textwidth}{0.4pt}\\
\bigskip
Correlatore\\
prof.\ Adriano PERON\\
\vspace{0.8cm}
\rule{0.6\textwidth}{0.4pt}
\end{flushleft}
\begin{flushright}
Dottorando \\
Alberto MOLINARI\\
\vspace{0.8cm}
\rule{0.6\textwidth}{0.4pt}
\end{flushright}
\end{large}

\vfill

\hrule
\bigskip
{\large Anno Accademico 2018/2019}
\end{center}

\end{minipage}
};%fine minipage
